Information Geometry of Message Passing

We show that the natural-gradient stationary condition of variational inference has an edge-local form on a Forney-style factor graph. We start from the Bethe free energy and constrain a selected edge marginal to an exponential family. At a stationary point, the natural parameter of that edge equals the sum of two projected messages, one from each incident factor. Each projected message is the natural-gradient projection of the exact belief-propagation log-message at the current receiving marginal, or equivalently, the gradient of its expectation in the so-called mean coordinates. We call the resulting scheme natural-gradient message passing (NGMP). The rule is local; each edge may carry its own exponential family, and the message a factor sends depends on the marginal that receives it. Compared with variational message passing, NGMP keeps the part of the exact message that the receiving family can represent instead of averaging the factor under the neighboring beliefs. The two coincide when the uncertainty on the edges entering a non-conjugate factor vanishes, and NGMP is more accurate when that uncertainty persists, for example, along a partially observed latent chain or when parameters are filtered through successive data batches. Experiments on Poisson smoothing, heteroskedastic regression, and hourly ETTh forecasting confirm this and show that the gain appears mainly in uncertainty calibration.

==> figures/factor-graphs/info-gem/ffg_styles.tex <==
% Shared TikZ styles for the Forney-style factor-graph figures.
% \input this file once at the top of each figure file, then start the
% picture with \begin{tikzpicture}[ffg].
%
% Edge styles encode variable roles (same convention in every figure):
%   solid      weights, features, observations
%   dashed     precisions
%   dash-dot   latent log-precision scores
\providecommand{\nexpsym}{\ensuremath{\mathcal N_{\!\exp}}}
\tikzset{
    ffg/.style={every node/.append style={font=\small}},
    paneltitle/.style={font=\bfseries\small, align=center},
    prior/.style={draw=black!70, fill=white, minimum width=8mm,
                  minimum height=6mm, inner sep=2pt},
    fact/.style={draw=black!70, fill=white, minimum width=8mm,
                 minimum height=7mm, inner sep=2pt},
    softfact/.style={fact, inner xsep=3pt},
    composite/.style={draw=black!70, double, double distance=1.2pt,
                      rounded corners=1pt, fill=white, minimum width=9mm,
                      minimum height=8mm, inner sep=1pt},
    eqfact/.style={draw=black!70, fill=white, minimum size=4.5mm,
                   inner sep=0pt},
    clamped/.style={rectangle, fill=black, draw=black, inner sep=0pt,
                    minimum size=1.8mm},
    port/.style={circle, draw=black!70, fill=white, inner sep=0pt,
                 minimum size=2.4mm},
    edge/.style={semithick, black!75},
    crossedge/.style={edge, preaction={draw=white, line width=2.8pt}},
    precisionedge/.style={edge, dashed},
    scoreedge/.style={edge, dash dot},
    forward/.style={edge, -{Latex[length=1.8mm]}},
    stopbar/.style={black!85, line width=1.05pt},
    edgelabel/.style={font=\scriptsize, fill=white, inner sep=1pt},
    portlabel/.style={font=\scriptsize},
    sublabel/.style={font=\scriptsize, text=black!65},
    fragment/.style={draw=black!50, dashed, rounded corners=1mm, semithick},
    batchframe/.style={draw=black!45, dashed, rounded corners=1mm, semithick},
}


==> figures/factor-graphs/info-gem/nexp_fragment.tex <==
% Opened \nexpsym composite with the softdot opened as well (box in a box):
% a deterministic dot product forms b^T phi, which a plain Gaussian receives
% as its mean; the Gaussian's precision is the exponentiated incoming score,
% tau = e^s.  Together the dot and N boxes are the softdot factor
% (eq:softdot-factor) drawn graphically.
%
% Ports: coefficients b (top), features phi (left, dot row), score in s
% (left, main row), output z (right).
%
% \input this inside a tikzpicture after defining
%     \coordinate (nexp-anchor) at ...;
% (the exp factor is centred on that coordinate).  Provides the nodes
% nexp-exp, nexp-norm, nexp-dot, nexp-sd, nexp-frag and the ports
% nexp-{s,b,phi,z}.
\node[fact] (nexp-exp) at (nexp-anchor) {$\exp$};
\node[fact] (nexp-norm) [right=15mm of nexp-exp] {$\mathcal N$};
\node[fact] (nexp-dot) [above=6mm of nexp-norm] {\texttt{dot}};
\draw[edge] (nexp-dot) --
    node[right=0.5mm, portlabel] {$b^{\!\top}\phi$} (nexp-norm);
\draw[precisionedge] (nexp-exp) --
    node[pos=0.32, above, edgelabel] {$\tau=e^{s}$} (nexp-norm);
% Inner box: the opened softdot.
\node[fragment, fit=(nexp-dot)(nexp-norm), inner xsep=3.5mm,
      inner ysep=2mm] (nexp-sd) {};
\node[font=\scriptsize\ttfamily, anchor=north, inner sep=1pt]
    (nexp-sdlab) at ($(nexp-sd.south)+(0,-0.7mm)$) {softdot};
% Outer box: the composite.
\node[fragment, fit=(nexp-exp)(nexp-sd)(nexp-sdlab), inner sep=3mm]
    (nexp-frag) {};
\node[anchor=south west, inner sep=1pt] at (nexp-frag.north west) {$\nexpsym$};
% Ports.
\node[port] (nexp-s) [left=7mm of nexp-exp] {};
\node[portlabel, left=0.5mm of nexp-s] {$s$};
\draw[scoreedge] (nexp-s) -- (nexp-exp);
\node[port] (nexp-b) [above=8mm of nexp-dot] {};
\node[portlabel, above=0.5mm of nexp-b] {$b$};
\draw[edge] (nexp-b) -- (nexp-dot);
\node[clamped] (nexp-phi) at ($(nexp-frag.west |- nexp-dot)+(-5mm,0)$) {};
\node[portlabel, left=0.5mm of nexp-phi] {$\phi$};
\draw[edge] (nexp-phi) -- (nexp-dot);
\node[port] (nexp-z) [right=8mm of nexp-norm] {};
\node[portlabel, right=0.5mm of nexp-z] {$z$};
\draw[scoreedge] (nexp-norm) -- (nexp-z);

